Deceiving End-to-End Deep Learning Malware Detectors using Adversarial Examples

In recent years, deep learning has shown performance breakthroughs in many applications, such as image detection, image segmentation, pose estimation, and speech recognition. However, this comes with a major concern: deep networks have been found to be vulnerable to adversarial examples. Adversarial examples are slightly modified inputs that are intentionally designed to cause a misclassification by the model. In the domains of images and speech, the modifications are so small that they are not seen or heard by humans, but nevertheless greatly affect the classification of the model. Deep learning models have been successfully applied to malware detection. In this domain, generating adversarial examples is not straightforward, as small modifications to the bytes of the file could lead to significant changes in its functionality and validity. We introduce a novel loss function for generating adversarial examples specifically tailored for discrete input sets, such as executable bytes. We modify malicious binaries so that they would be detected as benign, while preserving their original functionality, by injecting a small sequence of bytes (payload) in the binary file. We applied this approach to an end-to-end convolutional deep learning malware detection model and show a high rate of detection evasion. Moreover, we show that our generated payload is robust enough to be transferable within different locations of the same file and across different files, and that its entropy is low and similar to that of benign data sections.

==> preserving_functionality.tex <==
% !TEX root = main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% BENIGN CONFIDENCE %%%
%\begin{figure*}[h!]
%\centering
%\begin{subfigure}[t]{.5\textwidth}
%  \centering
%  \includegraphics[width=\linewidth]{figures/avg_conf}
%  \caption{Average of the confidence.}
%  \label{fig:avg_plot}
%\end{subfigure}%
%~~~
%\begin{subfigure}[t]{.5\textwidth}
%  \centering
%  \includegraphics[width=\linewidth]{figures/std_conf}
%  \caption{Standard deviation of the confidence.}
%  \label{fig:std_plot}
%\end{subfigure}
%\caption{The confidence of the class \emph{benign} as a function of the loss tradeoff parameter $\alpha$. The red and cyan lines present the confidence for $p=2$ and $p=\infty$, respectively.}\label{fig:confidence}
%\end{figure*}

%\begin{figure}[t!]
%\centering
%\vspace{-.6cm}
%\includegraphics[width=\linewidth]{figures/avg_conf}
%\caption{Average of the confidence.}
%\label{fig:avg_plot}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Preserving Functionality}
\label{payload_teaser}

So far we have discussed how to modify a binary file to cause misclassification.
%So far we have discussed how to modify the embedding vector and reconstruct a modified binary file.
However, utilizing this approach directly might not preserve the functionality of the file as the changes could affect the whole file.
We propose to contain modifications to a small chunk of bytes.
%We propose to create a small chunk of bytes that are crafted so as to cause misclassification of the whole file. The modifications are contained to this small chunk only. 
We refer to this chunk as the \emph{payload}.

This payload can be injected to the original file in one of two ways: 
(i) \emph{mid-file injection} -  the payload is placed in existing contingent unused bytes of sections where the physical size is greater than the virtual size;
(ii) \emph{end-of-file injection} - treating the payload as a new section and appending it to the file. Either approach would result in a valid and runnable code as the payload is inserted into non-executable code sections. We applied both methods and report results in \secref{sec:experiments}.

Algorithm~\ref{algo:adv} presents pseudo-code for generating a payload and injecting it at end-of-file. In this case, we append a uniformly random sequence of bytes of length $k$, $\smash{\x^{\text{payload}}\in\X^k}$, to the original file $\x$. We then embed the new binary $\smash{\x^{\text{new}}=[\x ; \x^{\text{payload}}]}$, to get $\smash{\z^{\text{new}}=[\z ; \z^{\text{payload}}]}$. Next, we iteratively perturb the appended segment $\smash{\z^{\text{payload}}}$ and stop when $\smash{f_\theta}$ misclassifies $\smash{\z^{\text{new}}}$. By perturbing only the appended segment, we ensure that $\z$ is kept intact and the functionality of $\x$ is preserved. This results in $\x^{\text{new}}$ that behaves identically to $\x$ but evades detection by $f_\theta$.
For the setting of mid-file injections we use the same perturbed payload $\smash{\x^{\text{payload}}}$ depicted in the previous paragraph, and inject it into contingent unused bytes where the physical size is greater than the virtual size. 
%Finding unused space is relatively easy as most binary files have physical and virtual size misalignments in their sections. Moreover, a malware creator can write the malware source code so that the executable will have sufficient unused space.
%The mid-file injection option results in a new binary file, with the same functionality as the original. Moreover, the original file's size is preserved, thus further obscuring any tampering with the file.

%\subsection{Properties}
%We describe some desirable properties of the generated payload. Such properties will increase the evasion rate, and make the detection of the payload harder. In \secref{payload_exp} we will present experimental results and further analysis. 
%
%\paragraph{Spatial Invariance} 
%We show a surprising property of the generated payload: the same generated payload can make a malicious binary file be misclassified as benign by both methods of injection (mid-file and end-of-file). This means that the generated payload is robust to shifting locations in the file, and can be successfully injected to multiple positions in a given file.
%
%\paragraph{File Transferability} 
%We show that an adversarial payload generated for a malicious binary file A can be injected to a different malicious binary file B. In most cases, this will cause file B to be misclassified as benign as well. This means that the generated payload is potent enough to be used across multiple files and multiple malware families.
%
%\paragraph{Payload Size} 
%Our payload size is extremely small (500-1000 bytes). This drastically increases the evasion rate for mid-file injection, as less unused bytes are required for the injection. For end-of-file injections this will result in a smaller change to the file size. 
%
%\paragraph{Entropy} 
%Entropy-based malware detectors identify malicious code sections by calculating their entropy \cite{lyda2007using}, and comparing to some standard threshold according to section type. Typically, a  higher entropy draws more suspicion. We show that our adversarial payload has low entropy, which is consistent with benign data sections. We also show that upon mid-file injections, the entropy of the section injected with the payload is practically unchanged.
%
%We conclude that it is not trivial to identify the location and size of the adversarial payload manually or automatically due to its varying length and location, and its inconspicuous entropy.


==> related_work.tex <==
% !TEX root = main.tex

\section{Related Work}
\label{sec:related}

\textbf{Learning-based Malware Detection. }
Machine learning and especially deep learning methods are  widely used for classification tasks in many fields such as computer vision~\cite{alexnet2012}, speech~\cite{DLacousticModeling2012} and natural language processing ~\cite{luong2015effective}, and typically achieve  state-of-the-art results. 

Previous machine learning based malware detection methods analyzed binary files using handcrafted features. Raff et al. ~\cite{raff2016investigation} represented the binary  by its n-grams. Sami et al. ~\cite{sami2010malware} used API calls to represent the binary. Yuan et al. \cite{yuan2014droid} performed static analysis of Android APK files using static and dynamic features. Azar et. al~\cite{yousefi2018malytics} presented an integrated system which extracts static features using locality sensitive hashing.
 
 Recent studies by Raff et~al.~\cite{Raff2017} and Kr{\v{c}}{\'a}l et~al.~\cite{krvcal2018deep} demonstrated effective malware detection systems, which are based on end-to-end CNN models. These systems analyze the raw data directly and utilize highly complex non-linear correlation between the raw bytes of the file to discriminate malicious and benign files. The end-to-end approach for classification has a substantial advantage -- no domain-knowledge is required about the task at hand. On the other hand, it was shown that for various tasks, end-to-end models are vulnerable to adversarial examples.
 In this work we will focus on such end-to-end systems \cite{Raff2017}.
 
\smallskip

\textbf{Adversarial Examples.}
There had been multiple studies in the area of adversarial examples. These studies showed that while end-to-end deep networks can achieve high performance on unknown input, they are vulnerable to small perturbations causing misclassification \cite{Fawzi2017robustness,carlini2017AE}. Additional studies have described how such adversarial examples can be crafted  \cite{goodfellow2015explaining}. Furthermore, Szegedy et al. \cite{szegedy2013properties} showed that adversarial examples can be generalized across models and datasets.
Cisse et al. \cite{HoudiniCISSE} introduced a novel flexible approach named Houdini for generating adversarial examples specifically tailored for the final performance measure of the task considered. Kreuk et al. \cite{kreuk2018fooling} investigated the generation of adversarial examples for attacking end-to-end neural based speaker verification models, and Carlini et al. \cite{carlini2016hidden} showed adversarial attack on a voice command system.

\smallskip

\textbf{Adversarial Examples for Malware. }Grosse et al.~\cite{GrossePMBM17} trained a neural network on a vector of features extracted from Android APK manifest files and appended additional features at the end of the manifest. Then, the algorithm described in \cite{papernot2016limitations} was used to craft adversarial examples.
Hu et al. \cite{hu2017black} proposed a generative adversarial network (GAN)-based approach. The work used binary indicator features representing API calls. Bogus API calls were simulated by switching binary indicator features when generating adversarial examples.
Xu et al. \cite{evademl} presented evasion techniques for malicious PDF files. The tree-like structure of PDFs makes them suitable for mutations based on genetic programming. The genetic programming procedure created mutated variations of the original PDF so as to evade detection.
Rosenberg et al. \cite{BGUrnn} created adversarial API call sequences to fool API based malware detectors.
While the above methods make use of hand-engineered features, our focus is the generation of adversarial examples for the case of raw binaries.
